Distributed Proximal Gradient Algorithm for Partially Asynchronous Computer Clusters

With ever growing data volume and model size, an error-tolerant, communication efficient, yet versatile distributed algorithm has become vital for the success of many large-scale machine learning applications. In this work we propose m-PAPG, an implementation of the flexible proximal gradient algorithm in model parallel systems equipped with the partially asynchronous communication protocol. The worker machines communicate asynchronously with a controlled staleness bound $s$ and operate at different frequencies. We characterize various convergence properties of m-PAPG: 1) Under a general non-smooth and non-convex setting, we prove that every limit point of the sequence generated by m-PAPG is a critical point of the objective function; 2) Under an error bound condition, we prove that the function value decays linearly for every $s$ steps; 3) Under the Kurdyka-${\L}$ojasiewicz inequality, we prove that the sequences generated by m-PAPG converge to the same critical point, provided that a proximal Lipschitz condition is satisfied.

==> related.tex <==
%!TEX root = main.tex

\section{Related Works}\label{sec:related}
%The stale synchronous parallel system of \mspg dates back to \cite{BT_parallel}, where it is also refered to as partially asyncrhonous parallel system. These work consider using stale synchronous systems to solving different kinds of optimizations problems with allowing machines to skip updates during the process. 
Asymptotic convergence of partially asynchronous gradient descent algorithm for solving unconstraint smooth optimizations is established in \cite{BT_parallel}, with its stochastic version being analyzed in \cite{BT_asy_gradient}. 
Asymptotic convergence of partially asynchronous gradient projection algorithm for solving smooth optimizations with convex constraint is established in  \cite{BT_parallel}, and a ``B-step" linear convergence is further established in \cite{Tseng_linear_PAA} with an error bound condition. Linear convergence of partially asynchronous algorithm for finding the fixed point of maximum norm contraction mappings is established in \cite{BT_asy, asy_iteration}.

Another series of work focus on SSP systems where machines are not allowed to operate at different paces \cite{LiMu_delay_pga, LiMu_delay_pga_coord, parameter_server}. In their settings, The system imposes an upper bound on the maximum clock difference between machines. Asymptotic convergence is established for proximal gradient algorithm for data parallelism \cite{LiMu_delay_pga} and for block coordinate descent \cite{LiMu_delay_pga_coord} with a smooth objective and convex regularizer. Other works consider stochastic algorithms on stale synchronous system. \cite{ssp_parameter} proposes an SSP system for stochastic gradient descent, and establishes $O(1/\sqrt{k})$ regret bound under bounded diameter and bounded sub-gradient assumption. 

\cite{delay_pga_linear, hogwild} consider a delayed stochastic gradient descent algorithm. Linear convergence to a neighborhood of optimum is established with strong convexity assumption in \cite{delay_pga_linear} and with additional bounded gradient assumption in \cite{hogwild}.  \cite{distrib_delay} proposes a distributed delayed dual averaging and mirror descent algorithm, and establishes $O(1/\sqrt{k})$ regret bound under standard stochastic assumptions. 


